Designing Electronic Markets for Defeasible-based Contractual Agents

The design of punishment policies applied to specific domains linking agents actions to material penalties is an open research issue. The proposed framework applies principles of contract law to set penalties: expectation damages, opportunity cost, reliance damages, and party design remedies. In order to decide which remedy provides maximum welfare within an electronic market, a simulation environment called DEMCA (Designing Electronic Markets for Contractual Agents) was developed. Knowledge representation and the reasoning capabilities of the agents are based on an extended version of temporal defeasible logic.

==> fig/producer_consumer <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 30 50 0 20 0.000 1 0.0000 5325 2400 150 150 5325 2400 5475 2400
1 3 0 1 0 30 50 0 -1 0.000 1 0.0000 7392 2406 150 150 7392 2406 7542 2406
2 4 0 1 0 30 50 0 20 0.000 0 0 8 0 0 5
	 4650 3044 4200 3044 4200 2775 4650 2775 4650 3044
2 4 0 1 0 7 50 0 -1 0.000 0 0 8 0 0 5
	 4575 2144 4575 1875 4125 1875 4125 2144 4575 2144
2 4 0 1 0 30 50 0 -1 0.000 0 0 9 0 0 5
	 6675 2550 6175 2550 6175 2250 6675 2250 6675 2550
2 2 0 1 0 30 50 0 -1 0.000 0 0 7 0 0 5
	 8025 1875 8400 1875 8400 2175 8025 2175 8025 1875
2 2 0 1 0 30 50 0 20 0.000 0 0 7 0 0 5
	 8025 2550 8400 2550 8400 2850 8025 2850 8025 2550
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3375 3150 4125 2925
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 4650 2850 5175 2550
2 1 0 1 0 30 50 0 20 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 7500 2325 8025 2025
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3375 3825 4275 3075
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 4575 1950 5175 2250
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3375 1650 4200 2775
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 5400 2475 8025 2700
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 5475 2325 6150 2325
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 6675 2400 7200 2400
4 0 0 50 0 0 14 0.0000 4 195 210 4275 2100 p4\001
4 0 0 50 0 0 14 0.0000 4 195 255 4275 3000  p5\001
4 0 0 50 0 0 14 0.0000 4 195 210 6300 2475 p6\001
4 0 0 50 0 0 14 0.0000 4 150 210 8100 2100 c1\001
4 0 0 50 0 0 14 0.0000 4 150 210 8100 2775 c2\001
4 0 0 50 0 0 14 0.0000 4 195 210 5250 2475 g6\001
4 0 0 50 0 0 14 0.0000 4 195 210 7275 2475 g7\001
4 0 0 50 0 0 12 0.0000 4 135 90 3975 2475 5\001
4 0 0 50 0 0 12 0.0000 4 135 180 3750 2925 10\001
4 0 0 50 0 0 12 0.0000 4 135 180 3750 3375 15\001
4 0 0 50 0 0 12 0.0000 4 135 180 4875 2925 32\001
4 0 0 50 0 0 12 0.0000 4 135 180 4875 2025 34\001
4 0 0 50 0 0 12 0.0000 4 135 180 5250 2175 34\001
4 0 0 50 0 0 12 0.0000 4 135 180 5850 2250 35\001
4 0 0 50 0 0 12 0.0000 4 135 180 6825 2850 37\001


==> fig/supplier_consumer <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 30 50 0 20 0.000 1 0.0000 1875 2175 168 168 1875 2175 2043 2175
1 3 0 1 0 30 50 0 20 0.000 1 0.0000 4275 2325 75 75 4275 2325 4350 2325
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 4275 1800 75 75 4275 1800 4200 1800
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 4875 2025 75 75 4875 2025 4800 2025
1 3 0 1 0 30 50 0 20 0.000 1 0.0000 4875 1200 75 75 4875 1200 4950 1200
2 2 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 600 2475 1125 2475 1125 2775 600 2775 600 2475
2 4 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 2550 1950 2550 1650 3000 1650 3000 1950 2550 1950
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1125 2550 1650 2250
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2550 1725 2100 2025
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2475 2550 2100 2325
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 3600 2700 5550 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 4575 2700 4575 975
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 2025 5550 2025
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1125 1800 1650 2100
2 2 0 1 0 30 50 0 15 0.000 0 0 -1 0 0 5
	 2550 2475 3000 2475 3000 2775 2550 2775 2550 2475
2 2 0 1 0 30 50 0 15 0.000 0 0 -1 0 0 5
	 600 1725 1125 1725 1125 2025 600 2025 600 1725
3 2 0 1 0 7 50 0 -1 0.000 0 1 1 3
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 4800 1200 4425 1725 4275 2250
	 0.000 -1.000 0.000
4 0 0 50 0 0 12 0.0000 4 180 180 2700 1875 p5\001
4 0 0 50 0 0 12 0.0000 4 135 180 1350 2700 13\001
4 0 0 50 0 0 12 0.0000 4 135 180 2250 1725 12\001
4 0 0 50 0 0 12 0.0000 4 135 180 2250 2700 15\001
4 0 0 50 0 0 12 0.0000 4 135 180 4350 2175 12\001
4 0 0 50 0 0 12 0.0000 4 135 180 4350 2475 11\001
4 0 0 50 0 0 12 0.0000 4 135 225 4350 1875  13\001
4 0 0 50 0 0 12 0.0000 4 135 180 4425 1575 14\001
4 0 0 50 0 0 12 0.0000 4 135 180 4350 1350 15\001
4 0 0 50 0 0 12 0.0000 4 195 585 5325 1950 Cp=12$\001
4 0 0 50 0 0 12 0.0000 4 135 180 1800 1950 12\001
4 0 0 50 0 0 12 0.0000 4 135 180 1425 1950 11\001
4 0 0 50 0 0 12 0.0000 4 165 90 4425 1050 $\001
4 0 0 50 0 0 12 0.0000 4 135 435 5550 2850 Items\001
4 0 0 50 0 0 12 0.0000 4 135 645 4275 2925 -1         1\001
4 0 0 50 0 0 12 0.0000 4 135 180 750 2700 s6\001
4 0 0 50 0 0 12 0.0000 4 180 180 5025 1950 p5\001
4 0 0 50 0 0 12 0.0000 4 135 180 5025 1200 c3\001
4 0 0 50 0 0 12 0.0000 4 135 180 3975 1800 s6\001
4 0 0 50 0 0 12 0.0000 4 135 180 3975 2400 s5\001
4 0 0 50 0 0 12 0.0000 4 135 270 675 1950   s5\001
4 0 0 50 0 0 12 0.0000 4 135 180 2700 2700 c3\001
4 0 0 50 0 0 12 0.0000 4 180 180 1800 2175 g5\001


==> fig/supplier_producer <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 30 50 0 20 0.000 1 0.0000 5325 2400 150 150 5325 2400 5475 2400
1 3 0 1 0 30 50 0 20 0.000 1 0.0000 3300 1575 150 150 3300 1575 3450 1575
1 3 0 1 0 30 50 0 20 0.000 1 0.0000 3225 3900 150 150 3225 3900 3375 3900
1 3 0 1 0 30 50 0 20 0.000 1 0.0000 3150 3150 150 150 3150 3150 3300 3150
2 4 0 1 0 30 50 0 20 0.000 0 0 8 0 0 5
	 4650 3044 4200 3044 4200 2775 4650 2775 4650 3044
2 4 0 1 0 7 50 0 -1 0.000 0 0 8 0 0 5
	 4575 2144 4575 1875 4125 1875 4125 2144 4575 2144
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3375 3150 4125 2925
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 4650 2850 5175 2550
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3375 3825 4275 3075
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3375 1650 4200 2775
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3450 1575 4050 1875
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 4575 1950 5175 2250
2 2 0 1 0 30 50 0 20 0.000 0 0 7 0 0 5
	 525 2850 900 2850 900 3150 525 3150 525 2850
2 2 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 525 3750 900 3750 900 4050 525 4050 525 3750
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 900 3825 3075 3825
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 3375 3900 5100 3900
2 2 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 5100 3750 5475 3750 5475 4050 5100 4050 5100 3750
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 900 3000 3000 3750
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 5475 2400 5850 2400
4 0 0 50 0 0 14 0.0000 4 195 210 4275 2100 p4\001
4 0 0 50 0 0 14 0.0000 4 195 255 4275 3000  p5\001
4 0 0 50 0 0 14 0.0000 4 195 210 3225 1650 g3\001
4 0 0 50 0 0 14 0.0000 4 195 210 3150 3975 g5\001
4 0 0 50 0 0 14 0.0000 4 195 210 5250 2475 g6\001
4 0 0 50 0 0 14 0.0000 4 195 210 3075 3225 g4\001
4 0 0 50 0 0 12 0.0000 4 135 180 600 3075 s5\001
4 0 0 50 0 0 12 0.0000 4 135 180 600 3975 s6\001
4 0 0 50 0 0 12 0.0000 4 135 180 5250 3975 c3\001
4 0 0 50 0 0 12 0.0000 4 135 180 1575 3750 12\001
4 0 0 50 0 0 12 0.0000 4 135 180 1500 3150 10\001
4 0 0 50 0 0 12 0.0000 4 135 180 3825 3600 15\001
4 0 0 50 0 0 12 0.0000 4 135 180 4500 3900 13\001
4 0 0 50 0 0 12 0.0000 4 135 180 3675 3000 10\001
4 0 0 50 0 0 12 0.0000 4 135 90 3750 2100 5\001
4 0 0 50 0 0 12 0.0000 4 135 180 3150 3675 12\001
4 0 0 50 0 0 12 0.0000 4 135 90 3075 2925 9\001
4 0 0 50 0 0 12 0.0000 4 135 90 3225 1350 5\001
4 0 0 50 0 0 12 0.0000 4 135 180 4875 2625 32\001
4 0 0 50 0 0 12 0.0000 4 135 180 4800 2025 34\001
4 0 0 50 0 0 12 0.0000 4 135 180 5250 2175 34\001
4 0 0 50 0 0 12 0.0000 4 135 180 5700 2625 35\001


==> fig/task <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 1469 2056 150 150 1469 2056 1319 2056
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 1425 2925 150 150 1425 2925 1275 2925
1 3 0 1 0 30 50 0 20 0.000 1 0.0000 5325 2400 150 150 5325 2400 5475 2400
1 3 0 1 0 30 50 0 20 0.000 1 0.0000 7392 2406 150 150 7392 2406 7542 2406
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 1425 2925 150 150 1425 2925 1275 2925
1 3 0 1 0 30 50 0 20 0.000 1 0.0000 1425 2925 150 150 1425 2925 1575 2925
1 3 0 1 0 30 50 0 20 0.000 1 0.0000 3225 3900 150 150 3225 3900 3375 3900
1 3 0 1 0 30 50 0 20 0.000 1 0.0000 3150 3150 150 150 3150 3150 3300 3150
1 3 0 1 0 30 50 0 20 0.000 1 0.0000 3300 1575 150 150 3300 1575 3450 1575
2 2 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 525 1875 900 1875 900 2175 525 2175 525 1875
2 2 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 525 4125 900 4125 900 4425 525 4425 525 4125
2 2 0 1 0 30 50 0 20 0.000 0 0 7 0 0 5
	 525 1125 900 1125 900 1425 525 1425 525 1125
2 4 0 1 0 30 50 0 20 0.000 0 0 8 0 0 5
	 2625 3044 2175 3044 2175 2775 2625 2775 2625 3044
2 4 0 1 0 7 50 0 -1 0.000 0 0 9 0 0 5
	 2675 3600 2675 3300 2175 3300 2175 3600 2675 3600
2 4 0 1 0 7 50 0 -1 0.000 0 0 8 0 0 5
	 2625 2100 2625 1875 2175 1875 2175 2100 2625 2100
2 4 0 1 0 30 50 0 20 0.000 0 0 8 0 0 5
	 4650 3044 4200 3044 4200 2775 4650 2775 4650 3044
2 4 0 1 0 7 50 0 -1 0.000 0 0 8 0 0 5
	 4575 2144 4575 1875 4125 1875 4125 2144 4575 2144
2 4 0 1 0 30 50 0 20 0.000 0 0 9 0 0 5
	 6675 2550 6175 2550 6175 2250 6675 2250 6675 2550
2 2 0 1 0 30 50 0 20 0.000 0 0 7 0 0 5
	 8025 1875 8400 1875 8400 2175 8025 2175 8025 1875
2 2 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 8025 2550 8400 2550 8400 2850 8025 2850 8025 2550
2 2 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 8025 3300 8400 3300 8400 3600 8025 3600 8025 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 1
	 1275 2925
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 1575 2925 2175 2925
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 2625 2925 3000 3075
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3375 3150 4125 2925
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 4650 2850 5175 2550
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 5475 2400 6150 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 6675 2400 7200 2400
2 1 0 1 0 30 50 0 20 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 7500 2325 8025 2025
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3375 3825 4275 3075
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3375 1650 4200 2775
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 900 1350 3150 1575
2 1 0 1 0 30 50 0 20 0.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 900 3675 3075 3825
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 3
	1 1 1.00 60.00 120.00
	 900 2025 1275 2025 1350 2025
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 1650 2025 2175 1950
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 2625 2025 3150 3000
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 900 4275 3075 3900
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 2625 3450 3075 3225
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 1500 3000 2175 3450
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3450 1575 4050 1875
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 4575 1950 5175 2250
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 5400 2475 8025 2775
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	1 1 1.00 60.00 120.00
	 3375 3900 8025 3450
2 2 0 1 0 30 50 0 20 0.000 0 0 7 0 0 5
	 525 3525 900 3525 900 3825 525 3825 525 3525
2 2 0 1 0 30 50 0 20 0.000 0 0 7 0 0 5
	 525 2925 900 2925 900 3225 525 3225 525 2925
2 2 0 1 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 525 2325 900 2325 900 2625 525 2625 525 2325
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 900 3075 1275 3000
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 900 2475 1275 2850
4 0 0 50 0 0 12 0.0000 4 135 180 600 1350 s1\001
4 0 0 50 0 0 12 0.0000 4 135 180 600 2100 s2\001
4 0 0 50 0 0 12 0.0000 4 180 180 2325 2025 p1\001
4 0 0 50 0 0 12 0.0000 4 180 180 2325 3000 p2\001
4 0 0 50 0 0 12 0.0000 4 180 180 2325 3525 p3\001
4 0 0 50 0 0 14 0.0000 4 195 210 4275 2100 p4\001
4 0 0 50 0 0 14 0.0000 4 195 255 4275 3000  p5\001
4 0 0 50 0 0 14 0.0000 4 195 210 6300 2475 p6\001
4 0 0 50 0 0 14 0.0000 4 150 210 8100 2100 c1\001
4 0 0 50 0 0 14 0.0000 4 150 210 8100 2775 c2\001
4 0 0 50 0 0 14 0.0000 4 150 210 8100 3525 c3\001
4 0 0 50 0 0 12 0.0000 4 180 180 1350 2100 g1\001
4 0 0 50 0 0 14 0.0000 4 195 210 1350 3000 g2\001
4 0 0 50 0 0 14 0.0000 4 195 210 3225 1650 g3\001
4 0 0 50 0 0 14 0.0000 4 195 210 3150 3975 g5\001
4 0 0 50 0 0 14 0.0000 4 195 210 5250 2475 g6\001
4 0 0 50 0 0 14 0.0000 4 195 210 7275 2475 g7\001
4 0 0 50 0 0 14 0.0000 4 195 210 3075 3225 g4\001
4 0 0 50 0 0 12 0.0000 4 135 180 600 2550 s3\001
4 0 0 50 0 0 12 0.0000 4 135 180 600 3150 s4\001
4 0 0 50 0 0 12 0.0000 4 135 180 600 3750 s5\001
4 0 0 50 0 0 12 0.0000 4 135 180 600 4350 s6\001


==> fig/toulmin.latex <==
\setlength{\unitlength}{4144sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(4209,2544)(1024,-2728)
\thinlines
{\color[rgb]{0,0,0}\put(1036,-1501){\framebox(1845,1305){}}
}%
{\color[rgb]{0,0,0}\put(1171,-2671){\framebox(405,315){}}
}%
{\color[rgb]{0,0,0}\put(2206,-2671){\framebox(405,315){}}
}%
{\color[rgb]{0,0,0}\put(1276,-1981){\oval(210,210)[bl]}
\put(1276,-1921){\oval(210,210)[tl]}
\put(2506,-1981){\oval(210,210)[br]}
\put(2506,-1921){\oval(210,210)[tr]}
\put(1276,-2086){\line( 1, 0){1230}}
\put(1276,-1816){\line( 1, 0){1230}}
\put(1171,-1981){\line( 0, 1){ 60}}
\put(2611,-1981){\line( 0, 1){ 60}}
}%
{\color[rgb]{0,0,0}\put(1396,-2356){\vector( 0, 1){270}}
}%
{\color[rgb]{0,0,0}\put(2341,-2356){\vector( 0, 1){270}}
}%
{\color[rgb]{0,0,0}\put(1801,-1816){\vector( 0, 1){315}}
}%
{\color[rgb]{0,0,0}\put(3196,-2716){\framebox(990,360){}}
}%
{\color[rgb]{0,0,0}\put(4366,-2671){\framebox(855,315){}}
}%
{\color[rgb]{0,0,0}\put(3256,-1936){\oval(210,210)[bl]}
\put(3256,-1876){\oval(210,210)[tl]}
\put(5071,-1936){\oval(210,210)[br]}
\put(5071,-1876){\oval(210,210)[tr]}
\put(3256,-2041){\line( 1, 0){1815}}
\put(3256,-1771){\line( 1, 0){1815}}
\put(3151,-1936){\line( 0, 1){ 60}}
\put(5176,-1936){\line( 0, 1){ 60}}
}%
{\color[rgb]{0,0,0}\put(4186,-1096){\framebox(990,900){}}
}%
{\color[rgb]{0,0,0}\put(2881,-601){\vector( 1, 0){1305}}
}%
{\color[rgb]{0,0,0}\put(3511,-1771){\vector( 0, 1){1170}}
}%
{\color[rgb]{0,0,0}\put(3556,-2311){\vector( 0, 1){270}}
}%
{\color[rgb]{0,0,0}\put(4681,-2311){\vector( 0, 1){270}}
}%
\put(1261,-421){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Expected Profit}%
}}}
\put(1261,-646){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Opportunity Cost}%
}}}
\put(1261,-871){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Reliance}%
}}}
\put(1261,-1096){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Substitute}%
}}}
\put(1261,-1321){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Time of breach}%
}}}
\put(1306,-2041){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Data Relevation}%
}}}
\put(1216,-2581){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Law}%
}}}
\put(2251,-2626){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Law}%
}}}
\put(3241,-2581){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Training Set}%
}}}
\put(4411,-2581){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Algorithm}%
}}}
\put(4366,-871){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Remedy}%
}}}
\put(3151,-331){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Inference}%
}}}
\put(3151,-556){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Mechanism}%
}}}
\put(3241,-1996){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Inference Relevation}%
}}}
\end{picture}

